Diffusion-SS3D: Diffusion Model for Semi-supervised 3D Object Detection

Semi-supervised object detection is crucial for 3D scene understanding, efficiently addressing the limitation of acquiring large-scale 3D bounding box annotations. Existing methods typically employ a teacher-student framework with pseudo-labeling to leverage unlabeled point clouds. However, producing reliable pseudo-labels in a diverse 3D space still remains challenging. In this work, we propose Diffusion-SS3D, a new perspective of enhancing the quality of pseudo-labels via the diffusion model for semi-supervised 3D object detection. Specifically, we include noises to produce corrupted 3D object size and class label distributions, and then utilize the diffusion model as a denoising process to obtain bounding box outputs. Moreover, we integrate the diffusion model into the teacher-student framework, so that the denoised bounding boxes can be used to improve pseudo-label generation, as well as the entire semi-supervised learning process. We conduct experiments on the ScanNet and SUN RGB-D benchmark datasets to demonstrate that our approach achieves state-of-the-art performance against existing methods. We also present extensive analysis to understand how our diffusion model design affects performance in semi-supervised learning.

==> 4_4_Experiment_Detail.tex <==
% \subsection{Implementation Details.}

% % 
% In this work, we employ the PointNet++~\cite{qi2017pointnet++} as the encoder backbone and IoU-aware VoteNet~\cite{wang20213dioumatch} as our decoder architecture.
% % 
% Following the multiple detection heads design~\cite{sun2021sparse, chen2022diffusiondet}, the detection decoder is modified to consist of two cascading stages.

% % 
% In the pre-training phase, we only use labeled data wih a batch size of four is to train the diffusion model.
% % 
% The model is trained for 901 epochs at a learning rate of 0.005, with learning decay applied at the 400th, 600th, and 800th epochs, each at a rate of 0.1.
% % 
% During the SSL training stage, a batch is composed of four labeled and eight unlabeled data.
% % 
% The pre-trained model's weights are used for initializing both the teacher and student models.
% % 
% The student model is trained for 1,001 epochs using the AdamW optimizer, with an initial learning rate of 0.005.
% % 
% The learning rate decays at the 400th, 600th, 800th, and 900th epochs to 0.3, 0.3, 0.1, and 0.1, respectively.
% % 

% For the diffusion processing initialization, we set the maximum timesteps to 1000and the number of proposal boxes to 128.
% % 
% The size and center Signal-to-Noise Ratio (SNR) are set at 2.0, and the label SNR at 4.0.
% % 
% We note that during random sampling from the Gaussian distribution, the object may be inconspicuous, occupying only a small space in the 3D scene.
% % 
% Therefore, while DiffusionDet sets the sampled center and size's mean at 0.5, we propose a smaller value of 0.25 for our size's mean.
% % 
% The mean of random sampling for the diffusion label is adjusted to the reciprocal of the number of classes.

% % 
% We perform twice DDIM sampling~\cite{song2020denoising} within the teacher model to produce pseudo-labels, and also during the evaluation of the overall SSL results.
% % 
% For box renewal and the pseudo-label filteri ng, we apply three metrics as in~\cite{wang20213dioumatch}: an objectness score threshold at 0.9, a classification confidence score threshold at 0.9, and an estimated IoU score threshold at 0.25.
% % 
% Following~\cite{wang20213dioumatch, ho2022learning}, to ensure a fair comparison, we employ test-time IoU at an optimization rate of 0.0005.
% % 
%  All experiments are conducted on a single GTX 3090 GPU.

